Average skew information-based coherence and its typicality for random quantum states

We study the average skew information-based coherence for both random pure and mixed states. The explicit formulae of the average skew information-based coherence are derived and shown to be the functions of the dimension N of the state space. We demonstrate that as N approaches to infinity, the average coherence is 1 for random pure states, and a positive constant less than 1/2 for random mixed states. We also explore the typicality of average skew information-based coherence of random quantum states. Furthermore, we identify a coherent subspace such that the amount of the skew information-based coherence for each pure state in this subspace can be bounded from below almost always by a fixed number that is arbitrarily close to the typical value of coherence.

==> DH_preamble.tex <==
%-----------------------------------------------------------------------------%
% Lin Chen's environment:



%6=journal
\newcommand{\aop}{Ann. Phys.~}
\newcommand{\cmp}{Comm. Math. Phys.~}
\newcommand{\ieee}{IEEE. Trans. Inf. Theory~}
\newcommand{\jmp}{J. Math. Phys.~}
\newcommand{\jpa}{J. Phys. A~}
\newcommand{\lmp}{Lett. Math. Phys.~}
\newcommand{\natpho}{Nat. Photon.~}
\newcommand{\natphy}{Nature Phys.~}
\newcommand{\natl}{Nature (London)~}
\newcommand{\njp}{New. J. Phys.~}
\newcommand{\phyr}{Phys. Rep.~}
\newcommand{\prl}{Phys. Rev. Lett.~}
\newcommand{\pra}{Phys. Rev. A~}
\newcommand{\pla}{Phys. Lett. A~}
\newcommand{\rmp}{Rev. Math. Phys.~}
\newcommand{\sci}{Science}
\newcommand{\laa}{Lin. Alg. App.~}

%-----------------------------------------------------------------------------%
% Fonts:
%-----------------------------------------------------------------------------%

\usepackage{appendix}
\usepackage{epstopdf}
\usepackage{color}
\usepackage{subfigure}
\usepackage[T1]{fontenc}
\usepackage[sc]{mathpazo}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx,color}
\usepackage{framed}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{amsthm}% theorems and proofs
\usepackage{amsfonts,mathrsfs}
\usepackage{geometry} % allows easy specifying of the page layout
\usepackage{eepic}
\usepackage{ifthen}
\usepackage[vcentermath]{youngtab}
\usepackage[unicode=true,pdfusetitle, bookmarks=true,bookmarksnumbered=false,bookmarksopen=false, breaklinks=false,pdfborder={0 0 0},backref=false,colorlinks=false] {hyperref}
\hypersetup{
colorlinks,linkcolor=myurlcolor,citecolor=myurlcolor,urlcolor=myurlcolor}
\definecolor{myurlcolor}{rgb}{0,0,0.7}% Color highlighted for numbers in citations and theorems

\geometry{
  verbose,
  dvips,
  width=422.695pt, marginparsep=0pt, marginparwidth=0pt,
  top=72.27pt, headheight=12pt, headsep=36pt, footskip=30pt, bottom=72.27pt
}

%-----------------------------------------------------------------------------%
% Colors:
%-----------------------------------------------------------------------------%

\usepackage{color}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\tbc}{\red{TO BE CONTINUED...}}
\newcommand{\opp}{\red{OPEN PROBLEMS}.~}
\newcommand{\proj}[1]{| #1\rangle\!\langle #1 |}
\newcommand{\ketbra}[2]{|#1\rangle\!\langle#2|}

%-----------------------------------------------------------------------------%
% Margins:
%-----------------------------------------------------------------------------%

\setlength{\topmargin}{0in} \setlength{\headheight}{0in}
\setlength{\headsep}{0.0in} \setlength{\textheight}{8.85in}
\setlength{\oddsidemargin}{0in} \setlength{\evensidemargin}{0in}
\setlength{\textwidth}{6.5in}

%-----------------------------------------------------------------------------%
% PDF:
%-----------------------------------------------------------------------------%

\usepackage{hyperref}
\hypersetup{pdfpagemode=UseNone}

%-----------------------------------------------------------------------------%
% Macros:
%-----------------------------------------------------------------------------%

\newcommand{\comment}[1]{\begin{quote}\sf [*** #1 ***]\end{quote}}
\newcommand{\tinyspace}{\mspace{1mu}}
\newcommand{\microspace}{\mspace{0.5mu}}
\newcommand{\op}[1]{\operatorname{#1}}

\newcommand{\abs}[1]{\left\lvert\tinyspace #1 \tinyspace\right\rvert}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\norm}[1]{\left\lVert\tinyspace #1 \tinyspace\right\rVert}
\newcommand{\triplenorm}[1]{
  \left|\!\microspace\left|\!\microspace\left| #1
  \right|\!\microspace\right|\!\microspace\right|}

\renewcommand{\det}{\operatorname{det}}
\renewcommand{\t}{{\scriptscriptstyle\mathsf{T}}}
\newcommand{\ip}[2]{\left\langle #1 , #2\right\rangle}
\newcommand{\sip}[2]{\langle #1 , #2\rangle}
\newcommand{\fid}{\operatorname{F}}
\newcommand{\setft}[1]{\mathrm{#1}}
\newcommand{\lin}[1]{\setft{L}\left(#1\right)}
\newcommand{\density}[1]{\setft{D}\left(#1\right)}
\newcommand{\unitary}[1]{\setft{U}\left(#1\right)}
\newcommand{\trans}[1]{\setft{T}\left(#1\right)}
\newcommand{\channel}[1]{\setft{C}\left(#1\right)}
\newcommand{\herm}[1]{\setft{Herm}\left(#1\right)}
\newcommand{\pos}[1]{\setft{Pos}\left(#1\right)}
\newcommand{\pd}[1]{\setft{Pd}\left(#1\right)}
\newcommand{\sep}[1]{\setft{Sep}\left(#1\right)}
\newcommand{\sepd}[1]{\setft{SepD}\left(#1\right)}
\newcommand{\ppt}[1]{\setft{PPT}\left(#1\right)}
\newcommand{\sphere}[1]{\setft{S}\left(#1\right)}
\newcommand{\opset}[3]{\setft{#1}_{#2}\left(#3\right)}
\renewcommand{\vec}{\op{vec}}
\newcommand{\im}{\op{im}}
\newcommand{\rank}{\op{rank}}
\newcommand{\spn}{\op{span}}
\newcommand{\sign}{\op{sign}}
\newcommand{\reg}[1]{\mathsf{#1}}
\newcommand{\supp}{{\operatorname{supp}}} \newcommand{\var}{\operatorname{Var}}
\newcommand{\expect}{\operatorname{E}}
\def\locc{\text{LOCC}}
\def\per{\mathrm{Per}}
\def\alg{\mathrm{Alg}}
\def\comm{\mathrm{Comm}}
\def\gl{\mathfrak{gl}}
\def\u{\mathfrak{u}}
\def\g{\mathfrak{g}}
\def\h{\mathfrak{h}}
\def\k{\mathfrak{k}}
\def\n{\mathfrak{n}}
\def\liet{\mathfrak{t}}
\def\su{\mathfrak{su}}
\def\so{\mathfrak{so}}
\def\sl{\mathfrak{sl}}
\def\sp{\mathfrak{sp}}
\def\Ad{\mathrm{Ad}}
\def\ad{\mathrm{ad}}
\def\vol{\mathrm{vol}}
\def\dh{\mathrm{DH}}
\def\liel{\mathfrak{l}}

\def \dif {\mathrm{d}}
\def \diag {\mathrm{diag}}
\def \vol {\mathrm{vol}}
\def \re {\mathrm{Re}}
\def \im {\mathrm{Im}}

\def\complex{\mathbb{C}}
\def\real{\mathbb{R}}
\def\natural{\mathbb{N}}
\def\integer{\mathbb{Z}}
\def\I{\mathbb{1}}
\def \lket {\left|}
\def \rket {\right\rangle}
\def \lbra {\left\langle}
\def \rbra {\right|}

\newenvironment{mylist}[1]{\begin{list}{}{
    \setlength{\leftmargin}{#1}
    \setlength{\rightmargin}{0mm}
    \setlength{\labelsep}{2mm}
    \setlength{\labelwidth}{8mm}
    \setlength{\itemsep}{0mm}}}
    {\end{list}}

\renewcommand{\baselinestretch}{1.3}


%======================================================================================================================

\def\ot{\otimes}
\def\CP{\mathrm{CP}}
\newcommand{\inner}[2]{\langle #1 , #2\rangle}
\newcommand{\iinner}[2]{\langle #1 | #2\rangle}
\newcommand{\out}[2]{| #1\rangle\langle #2 |}
\newcommand{\Inner}[2]{\left\langle #1 , #2\right\rangle}
\newcommand{\Innerm}[3]{\left\langle #1 \left| #2 \right| #3 \right\rangle}
\newcommand{\defeq}{\stackrel{\smash{\textnormal{\tiny def}}}{=}}
\newcommand{\cls}[1]{\mathrm{#1}}
\newcommand{\Herm}{\mathrm{Herm}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\OT}[2]{#1 \otimes #2}

%======================================================================================================================

% parentheses, brakets, and sets
\newcommand{\pa}[1]{(#1)}
\newcommand{\Pa}[1]{\left(#1\right)}
\newcommand{\br}[1]{[#1]}
\newcommand{\Br}[1]{\left[#1\right]}
%\newcommand{\br}[1]{\pa{#1}}
%\newcommand{\Br}[1]{\Pa{#1}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}

%=======================================================================================================================

%Dirac notation
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\Bra}[1]{\left\langle#1\right|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\Ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[1]{\langle#1\rangle}
\newcommand{\Braket}[1]{\left\langle#1\right\rangle}

%=======================================================================================================================

% the Choi-Jamiolkowski isomorphism
%\DeclareMathOperator{\Jamiolkowski}{J}
\def\Jamiolkowski{J}
\newcommand{\jam}[1]{\Jamiolkowski\pa{#1}}
\newcommand{\Jam}[1]{\Jamiolkowski\Pa{#1}}


%=======================================================================================================================

% the matrix-vector correspondence
%\newcommand{\col}[1]{|#1\rangle}
%\newcommand{\row}[1]{\langle#1|}
%\newcommand{\Col}[1]{\left|#1\right\rangle}
%\newcommand{\Row}[1]{\left\langle#1\right|}
\DeclareMathOperator{\vectorize}{vec}
\newcommand{\col}[1]{\vectorize\pa{#1}}
\newcommand{\row}[1]{\vectorize\pa{#1}^{\dagger}}
\newcommand{\Col}[1]{\vectorize\Pa{#1}}
\newcommand{\Row}[1]{\vectorize\Pa{#1}^{\dagger}}

% the trace of an operator/matrix
\DeclareMathOperator{\trace}{Tr}
\newcommand{\ptr}[2]{\trace_{#1}\pa{#2}}
\newcommand{\Ptr}[2]{\trace_{#1}\Pa{#2}}
\newcommand{\tr}[1]{\ptr{}{#1}}
\newcommand{\Tr}[1]{\Ptr{}{#1}}

%=======================================================================================================================

% Norms
\newcommand{\Abs}[1]{\left|\tinyspace#1\tinyspace\right|}
\newcommand{\Norm}[1]{\left\lVert\tinyspace#1\tinyspace\right\rVert}
\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\Fnorm}[1]{\Norm{#1}_{\mathrm{F}}}
\newcommand{\tnorm}[1]{\norm{#1}_{\trace}}
\newcommand{\Tnorm}[1]{\Norm{#1}_{\trace}}
\newcommand{\dnorm}[1]{\norm{#1}_{\diamond}}
\newcommand{\Dnorm}[1]{\Norm{#1}_{\diamond}}
\newcommand{\snorm}[2]{\norm{#1}_{\diamond{#2}}}
\newcommand{\Snorm}[2]{\Norm{#1}_{\diamond{#2}}}

%=======================================================================================================================

% Fonts
\newcommand{\fontmapset}{\mathbf} % sets of mappings
\newcommand{\hilb}{\mathcal}      % Hilbert spaces

%=======================================================================================================================

% Sets of operators
\newcommand{\mset}[2]{\fontmapset{#1}\pa{#2}}
\newcommand{\Mset}[2]{\fontmapset{#1}\Pa{#2}}
\newcommand{\Lin}[1]{\Mset{L}{#1}}
\newcommand{\her}[1]{\mset{H}{#1}}
\newcommand{\Her}[1]{\Mset{H}{#1}}
\newcommand{\Pos}[1]{\Mset{H^+}{#1}}
%\newcommand{\tp} [2]{\mset{TP}{#1 \to #2}}
%\newcommand{\TP} [2]{\Mset{TP}{#1 \to #2}}

%=======================================================================================================================

% the Identity super-operator
\newcommand{\identity}{\mathbbm{1}}
%\newcommand{\idsup}[1]{\identity_{\lin{#1}}}
\newcommand{\idsup}[1]{\identity_{#1}}



%=======================================================================================================================
% Hilbert space shortcuts

\def\cA{\mathcal{A}}\def\cB{\mathcal{B}}\def\cC{\mathcal{C}}\def\cD{\mathcal{D}}\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}\def\cG{\mathcal{G}}\def\cH{\mathcal{H}}\def\cI{\mathcal{I}}\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}\def\cL{\mathcal{L}}\def\cM{\mathcal{M}}\def\cN{\mathcal{N}}\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}\def\cQ{\mathcal{Q}}\def\cR{\mathcal{R}}\def\cS{\mathcal{S}}\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}\def\cV{\mathcal{V}}\def\cW{\mathcal{W}}\def\cX{\mathcal{X}}\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

%=======================================================================================================================

\def\bA{\mathbf{A}}\def\bB{\mathbf{B}}\def\bC{\mathbf{C}}\def\bD{\mathbf{D}}\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}\def\bG{\mathbf{G}}\def\bH{\mathbf{H}}\def\bI{\mathbf{I}}\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}\def\bL{\mathbf{L}}\def\bM{\mathbf{M}}\def\bN{\mathbf{N}}\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}\def\bQ{\mathbf{Q}}\def\bR{\mathbf{R}}\def\bS{\mathbf{S}}\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}\def\bV{\mathbf{V}}\def\bW{\mathbf{W}}\def\bX{\mathbf{X}}\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}
%=======================================================================================================================

\def\bsA{\boldsymbol{A}}\def\bsB{\boldsymbol{B}}\def\bsC{\boldsymbol{C}}\def\bsD{\boldsymbol{D}}\def\bsE{\boldsymbol{E}}
\def\bsF{\boldsymbol{F}}\def\bsG{\boldsymbol{G}}\def\bsH{\boldsymbol{H}}\def\bsI{\boldsymbol{I}}\def\bsJ{\boldsymbol{J}}
\def\bsK{\boldsymbol{K}}\def\bsL{\boldsymbol{L}}\def\bsM{\boldsymbol{M}}\def\bsN{\boldsymbol{N}}\def\bsO{\boldsymbol{O}}
\def\bsP{\boldsymbol{P}}\def\bsQ{\boldsymbol{Q}}\def\bsR{\boldsymbol{R}}\def\bsS{\boldsymbol{S}}\def\bsT{\boldsymbol{T}}
\def\bsU{\boldsymbol{U}}\def\bsV{\boldsymbol{V}}\def\bsW{\boldsymbol{W}}\def\bsX{\boldsymbol{X}}\def\bsY{\boldsymbol{Y}}
\def\bsZ{\boldsymbol{Z}}
%=======================================================================================================================

\def\bsa{\boldsymbol{a}}\def\bsb{\boldsymbol{b}}\def\bsc{\boldsymbol{c}}\def\bsd{\boldsymbol{d}}\def\bse{\boldsymbol{e}}
\def\bsf{\boldsymbol{f}}\def\bsg{\boldsymbol{g}}\def\bsh{\boldsymbol{h}}\def\bsi{\boldsymbol{i}}\def\bsj{\boldsymbol{j}}
\def\bsk{\boldsymbol{k}}\def\bsl{\boldsymbol{l}}\def\bsm{\boldsymbol{m}}\def\bsn{\boldsymbol{n}}\def\bso{\boldsymbol{o}}
\def\bsp{\boldsymbol{p}}\def\bsq{\boldsymbol{q}}\def\bsr{\boldsymbol{r}}\def\bss{\boldsymbol{s}}\def\bst{\boldsymbol{t}}
\def\bsu{\boldsymbol{u}}\def\bsv{\boldsymbol{v}}\def\bsw{\boldsymbol{w}}\def\bsx{\boldsymbol{x}}\def\bsy{\boldsymbol{y}}
\def\bsz{\boldsymbol{z}}

%=======================================================================================================================

\def\ba{\mathbf{a}}\def\bb{\mathbf{b}}\def\bc{\mathbf{c}}\def\bd{\mathbf{d}}\def\be{\mathbf{e}}
\def\bff{\mathbf{f}}\def\bg{\mathbf{g}}\def\bh{\mathbf{h}}\def\bi{\mathbf{i}}\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}\def\bl{\mathbf{l}}\def\bm{\mathbf{m}}\def\bn{\mathbf{n}}\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}\def\bq{\mathbf{q}}\def\br{\mathbf{r}}\def\bs{\mathbf{s}}\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}\def\bv{\mathbf{v}}\def\bw{\mathbf{w}}\def\bx{\mathbf{x}}\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

%=======================================================================================================================

\def\rA{\mathrm{A}}\def\rB{\mathrm{B}}\def\rC{\mathrm{C}}\def\rD{\mathrm{D}}\def\rE{\mathrm{E}}
\def\rF{\mathrm{F}}\def\rG{\mathrm{G}}\def\rH{\mathrm{H}}\def\rI{\mathrm{I}}\def\rJ{\mathrm{J}}
\def\rK{\mathrm{K}}\def\rL{\mathrm{L}}\def\rM{\mathrm{M}}\def\rN{\mathrm{N}}\def\rO{\mathrm{O}}
\def\rP{\mathrm{P}}\def\rQ{\mathrm{Q}}\def\rR{\mathrm{R}}\def\rS{\mathrm{S}}\def\rT{\mathrm{T}}
\def\rU{\mathrm{U}}\def\rV{\mathrm{V}}\def\rW{\mathrm{W}}\def\rX{\mathrm{X}}\def\rY{\mathrm{Y}}
\def\rZ{\mathrm{Z}}

%=======================================================================================================================

\def\sA{\mathscr{A}}\def\sB{\mathscr{B}}\def\sC{\mathscr{C}}\def\sD{\mathscr{D}}\def\sE{\mathscr{E}}
\def\sF{\mathscr{F}}\def\sG{\mathscr{G}}\def\sH{\mathscr{H}}\def\sI{\mathscr{I}}\def\sJ{\mathscr{J}}
\def\sK{\mathscr{K}}\def\sL{\mathscr{L}}\def\sM{\mathscr{M}}\def\sN{\mathscr{N}}\def\sO{\mathscr{O}}
\def\sP{\mathscr{P}}\def\sQ{\mathscr{Q}}\def\sR{\mathscr{R}}\def\sS{\mathscr{S}}\def\sT{\mathscr{T}}
\def\sU{\mathscr{U}}\def\sV{\mathscr{V}}\def\sW{\mathscr{W}}\def\sX{\mathscr{X}}\def\sY{\mathscr{Y}}
\def\sZ{\mathscr{Z}}

%=======================================================================================================================

\def\A{\textsf{A}}\def\B{\textsf{B}}\def\C{\textsf{C}}\def\D{\textsf{D}}\def\E{\textsf{E}}
\def\F{\textsf{F}}\def\G{\textsf{G}}\def\H{\textsf{H}}                  \def\J{\textsf{J}}
\def\K{\textsf{K}}\def\L{\textsf{L}}\def\M{\textsf{M}}\def\N{\textsf{N}}\def\O{\textsf{O}}
\def\P{\textsf{P}}\def\Q{\textsf{Q}}\def\R{\textsf{R}}\def\S{\textsf{S}}\def\T{\textsf{T}}
\def\U{\textsf{U}}\def\V{\textsf{V}}\def\W{\textsf{W}}\def\X{\textsf{X}}\def\Y{\textsf{Y}}
\def\Z{\textsf{Z}}

%=======================================================================================================================

\def\mA{\mathbb{A}}\def\mB{\mathbb{B}}\def\mC{\mathbb{C}}\def\mD{\mathbb{D}}\def\mE{\mathbb{E}}
\def\mF{\mathbb{F}}\def\mG{\mathbb{G}}\def\mH{\mathbb{H}}                  \def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}\def\mL{\mathbb{L}}\def\mM{\mathbb{M}}\def\mN{\mathbb{N}}\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}\def\mQ{\mathbb{Q}}\def\mR{\mathbb{R}}\def\mS{\mathbb{S}}\def\mT{\mathbb{T}}
\def\mU{\mathbb{U}}\def\mV{\mathbb{V}}\def\mW{\mathbb{W}}\def\mX{\mathbb{X}}\def\mY{\mathbb{Y}}
\def\mZ{\mathbb{Z}}

%=======================================================================================================================

\newtheorem{thrm}{Theorem}[section]
\newtheorem{lem}[thrm]{Lemma}
\newtheorem{prop}[thrm]{Proposition}
\newtheorem{cor}[thrm]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[thrm]{Definition}
\newtheorem{remark}[thrm]{Remark}
\newtheorem{exam}[thrm]{Example}
\newtheorem{conj}[thrm]{Conjecture}
\numberwithin{equation}{section}

%-----------------------------------------------------------------------------%
% Question environment:
%-----------------------------------------------------------------------------%

\newcounter{questionnumber}
\newenvironment{question}
       {\begin{mylist}{\parindent}
     \item[\stepcounter{questionnumber}\thequestionnumber.]}
       {\end{mylist}}

